JACC: An OpenACC Runtime Framework with Kernel-Level and Multi-GPU Parallelization

The rapid development in computing technology has paved the way for directive-based programming models towards a principal role in maintaining software portability of performance-critical applications. Efforts on such models involve a least engineering cost for enabling computational acceleration on multiple architectures while programmers are only required to add meta information upon sequential code. Optimizations for obtaining the best possible efficiency, however, are often challenging. The insertions of directives by the programmer can lead to side-effects that limit the available compiler optimization possible, which could result in performance degradation. This is exacerbated when targeting multi-GPU systems, as pragmas do not automatically adapt to such systems, and require expensive and time consuming code adjustment by programmers. This paper introduces JACC, an OpenACC runtime framework which enables the dynamic extension of OpenACC programs by serving as a transparent layer between the program and the compiler. We add a versatile code-translation method for multi-device utilization by which manually-optimized applications can be distributed automatically while keeping original code structure and parallelism. We show in some cases nearly linear scaling on the part of kernel execution with the NVIDIA V100 GPUs. While adaptively using multi-GPUs, the resulting performance improvements amortize the latency of GPU-to-GPU communications.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

main.pdf: main.tex abstract.tex conc.tex background.tex results.tex method.tex intro.tex jacc.tex related.tex multigpu.tex acks.tex $(PACKAGE).cls main.bib fig/*
	pdflatex $<
	bibtex $(notdir $(basename $<))
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' main.log) \
	do pdflatex $<; done

%.cls:   %.ins %.dtx
	pdflatex $<

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

clean:
	$(RM)  *.log *.aux *.pdf \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \

distclean: clean

